Top-k Querying of Unknown Values under Order Constraints (Extended Version)

Many practical scenarios make it necessary to evaluate top-k queries over data items with partially unknown values. This paper considers a setting where the values are taken from a numerical domain, and where some partial order constraints are given over known and unknown values: under these constraints, we assume that all possible worlds are equally likely. Our work is the first to propose a principled scheme to derive the value distributions and expected values of unknown items in this setting, with the goal of computing estimated top-k results by interpolating the unknown values from the known ones. We study the complexity of this general task, and show tight complexity bounds, proving that the problem is intractable, but can be tractably approximated. We then consider the case of tree-shaped partial orders, where we show a constructive PTIME solution. We also compare our problem setting to other top-k definitions on uncertain data.

==> apx_prelim.tex <==
Denote by $G$ the directed graph on $\calX$ defined by the order constraints of $\calC$.
We compute in PTIME the directed acyclic graph $G'$ of the strongly connected components of $G$.

If $G$ contains two vertices $x$ and $y$ in the same connected component that have exact-value constraints to two values $v_x \neq v_y$, we claim that the admissible polytope is empty. Indeed, assuming without loss of generality that $v_x < v_y$,
considering the sequence of comparability relations
$y = x_1 \leq x_2  \leq \cdots \leq x_n = x$
(either in $\leq_{\calC}$ or implied by the exact-value constraints)
that was used to justify the existence of a path from $y$ to $x$,
any possible world in the admissible polytope would have to satisfy these order constraints,
which is impossible as $v_x < v_y$ and the value of $x$ and $y$ in the possible world must be $v_x$ and $v_y$ respectively.

If there are no two such vertices, we set the value of each strongly
connected component in $G'$ to be undefined if none of its nodes has an exact-value constraint,
or to be the value of the exact-value constraint of its nodes, if any.
(By the previous paragraph, there is at most one such value.)
If there are two strongly connected components $s$, $s'$ such that $s'$ is reachable from $s$ in $G'$ but the value of $s$ in $G'$ is strictly greater than the value of $s'$,
we claim that the admissible polytope is empty.
Indeed, considering a path of comparability relations from the node of $s$ with
an exact-value constraint
to the node of $s'$ with an exact-value constraint,
if we assume the existence of a possible world,
we reach a contradiction like before.

Otherwise, we claim that the admissible polytope is non-empty.
This is easily checked by completing the values assigned to nodes in~$G'$
so that all nodes have a value and no order constraint is violated,
and extending this to a possible world of $\calC$.


==> apx_ties.tex <==
\label{apx:ties}
We first define formally the notion of tied values.

\begin{definition}
  Given a constraint set $\calC$, we say that $x$ and $y$ have a
  \deft{persistent tie} if $\calC$ contains $x \leq y$ and $y \leq
  x$. (Remember that $\calC$ is closed under implication; so in particular $x$
  and $y$ have a persistent tie if they have an exact-value constraint to the
  same value.)

  We write $x \ptie y$ if $x$ and $y$ have a persistent tie. It is immediate
  that $\ptie$ is an equivalence relation.

  We say that $\calC$ has a \deft{persistent tie}
  if there are $x \neq y$ such that $x \ptie y$.
\end{definition}

\begin{lemma}
\label{lem:zeromass}
For any constraint set $\calC$ which has no persistent tie, the mass under the
uniform distribution of possible worlds with ties is $0$.
\end{lemma}

\begin{proof}
	\scream{[R3] clarify (``I am not sure what the authors mean by...'')}
  Let $d$ be the dimension of $\pw(\calC)$ and $n \defeq \card{\calX}$.
  Let $W$ be the subset of $\pw(\calC)$ of the possible worlds that have ties.
  We write $W$ as $\bigcup_{\substack{x_i, x_j \in \calX\\i \neq j}} W_{i, j}$,
  where $W_{i, j}$ is the subset of $\pw(\calC)$ of the possible worlds where
  there is a tie between~$x_i$ and~$x_j$. We clearly have:
  \[
    \pvol_d(W) \leq \card{\calX}^2
    \max_{\substack{x_i, x_j \in \calX\\i \neq j}} \pvol_d(W_{i, j})
  \]
  Hence, it suffices to
  show that for any $x_i, x_j \in \calX$, $i \neq j$, $\pvol_d(W_{i, j}) = 0$.

  Hence, fix $x_i, x_j \in \calX$, $i \neq j$.
  Remember that we have assumed that we only consider constraint sets $\calC$
  such that $\pw(\calC)$ is non-empty. Because $\calC$ is closed under
  implication, it cannot be the case that $t_i = t_j$ in every possible world
  $\mathbf{t} \in \pw(\calC)$; otherwise this implies that the constraints $x_i
  \leq x_j$ and $x_j \leq x_i$ are implied by $\calC$, so they hold in~$\calC$,
  and $\calC$ has a persistent tie, contradicting our assumption. Thus
  $\pw(\calC)$ is a convex polytope of dimension~$d$ in $[0, 1]^n$ which is not
  included in the hyperplane defined by the equation $x_i = x_j$. We deduce that
  $W_{i,j}$, the projection of $\pw(\calC)$ to that hyperplane, has dimension
  $d-1$, so that its volume $\pvol_d(W_{i,j}) = \int_{W_{i,j}} \frac{\d
  \mu_d}{V_d(\calC)}$ is~$0$.
  This concludes the proof.
\end{proof}

In the situation with persistent ties, we observe that, informally, tied
variables
can be collapsed to single variables, so as to remove the persistent ties without
changing substantially the possible worlds and their probability. Formally:

\begin{definition}
We define $\quot{\calX}{\sim}$ as the set of equivalence classes of $\calX$ for
$\sim$, and we define $\quot{\calC}{\sim}$ to be the constraint set where every
occurrence of a variable $x_i$ of $\calX$ is replaced by the variable of
$\quot{\calX}{\sim}$ corresponding to its equivalence class.
\end{definition}

The following is immediate:

\begin{lemma}
  \label{lem:assume}
For any constraint set $\calC$ on variable set $\calX$ with uniform distribution
$p_u$, the constraint set $\quot{\calC}{\sim}$ is without persistent ties, can
be computed in PTIME, and there is a
bijection $f$ from $\pw(\calC)$ to $\pw(\quot{\calC}{\sim})$.
\end{lemma}

\begin{proof}
  The computation of $\quot{\calC}{\sim}$ can be performed by computing in PTIME
  the strongly connected components of the graph of the $\sim$ relation, which
  we can clearly compute in PTIME from $\calC$. The absence of persistent ties
  is by observing that any persistent tie in the quotient between $X_i$ and
  $X_j$ in $\quot{\calX}{\sim}$ would imply the existence of $x_i, x_i' \in X_i$ and
  $x_j, x_j' \in X_j$ such that $\calC$ contains $x_i \leq x_j$ and $x_j' \leq
  x_i'$, from which we deduce the existence of a persistent tie between $x_i$
  and $x_j$ as $\calC$ contains $x_j \leq x_j'$, $x_i' \leq x_i$ by definition
  of $x_i \sim x_i'$, $x_j \sim x_j'$, so that we should have identified $x_i$
  and $x_j$ when constructing $\quot{\calX}{\sim}$.

  The bijection between the possible worlds is obtained by mapping any possible
  world $\mathbf{t} \in \pw(\calC)$ to $\mathbf{t'}$ obtained by choosing, for
  every $X_i \in \quot{\calX}{\sim}$, the value $t'_i$ as $t_j$ such that $x_j
  \in X_i$. (The choice of representative does not matter as the definition of
  $\sim$ implies that $t_j = t_{j'}$  for every $\mathbf{t} \in \pw(\calC)$
  whenever $x_j \sim x_{j'}$.)
\end{proof}

We conclude by showing how problems on $\calC$ can be reduced to problems on
$\quot{\calC}{\sim}$, concluding the proof of Proposition~\ref{prp:noties}.

The interpolation problem for a variable $x_i$ on $\calC$ clearly reduces to
interpolation for variable $X_j$ on $\quot{\calC}{\sim}$.

The top-$k$ computation problem on $\calC$ for a selection predicate $\sigma$
reduces to the top-$k$ computation problem on $\quot{\calC}{\sim}$ for the
selection predicate $\sigma'$ that selects variables $X_i$ such that some $x_j
\in X_i$ is selected by $\sigma$. Given the top-$k$ result $(X_1, \ldots, X_k)$
on $\quot{\calC}{\sim}$, we rewrite it to the top-$k$ result on $\calC$ by
replacing each $X_i$ by all the variables $x_j \in X_i$ selected by $\sigma$
(there is at least one of them), and truncating to length~$k$.

